NTSEBENCH: Cognitive Reasoning Benchmark for Vision Language Models

Cognitive textual and visual reasoning tasks, including puzzles, series, and analogies, demand the ability to quickly reason, decipher, and evaluate patterns both textually and spatially. Due to extensive training on vast amounts of human-curated data, LLMs and VLMs excel in common-sense reasoning tasks, however still struggle with more complex reasoning that demands deeper cognitive understanding. We introduce NTSEBench, a new dataset designed to evaluate cognitive multi-modal reasoning and problem-solving skills of large models. The dataset contains 2728 multiple-choice questions, accompanied by a total of 4,642 images, categorized into 26 different types. These questions are drawn from the nationwide NTSE examination in India and feature a mix of visual and textual general aptitude challenges, designed to assess intelligence and critical thinking skills beyond mere rote learning. We establish baselines on the dataset using state-of-the-art LLMs and VLMs. To facilitate a comparison between open source and propriety models, we propose four distinct modeling strategies to handle different modalities -- text and images -- in the dataset instances.

==> table-composite-interleaving.tex <==

\begin{table}[!htp]\centering
\caption{Generated by Spread-LaTeX}\label{tab: }
\scriptsize
\begin{tabular}{lrrrrrrrrrrrrrr}\toprule
&Model &SER &ALP &ODO &ANA &COD &NUM &BLR &MTO &PUZ &SYL &STC &DAT \\\cmidrule{2-14}
&\multicolumn{13}{c}{Textbased data} \\\midrule
\multirow{6}{*}{Zero shot} &textonly\_gpt\_3.5\_turbo\_0125 &0.359683794466403 &0.326086956521739 &0.4 &0.517241379310344 &0.363636363636363 &0.253623188405797 &0.365079365079365 &0.275510204081632 &0.463414634146341 &0.351351351351351 &0.403846153846153 &0.321428571428571 \\
&gpt\_4o &0.42578125 &0.351063829787234 &0.558823529411764 &0.655629139072847 &0.382550335570469 &0.424460431654676 &0.682539682539682 &0.414141414141414 &0.694736842105263 &0.636363636363636 &0.701923076923076 &0.433333333333333 \\
&gemini\_1.5\_flash &0.36328125 &0.223404255319148 &0.488235294117647 &0.569536423841059 &0.382550335570469 &0.39568345323741 &0.547619047619047 &0.404040404040404 &0.6 &0.636363636363636 &0.653846153846153 &0.422222222222222 \\
&textonly\_mixtral\_8x7b\_32768 &0.197628458498023 &0.195652173913043 &0.247058823529411 &0.455172413793103 &0.147727272727272 &0.268115942028985 &0.293650793650793 &0.295918367346938 &0.329268292682926 &0.243243243243243 &0.538461538461538 &0.333333333333333 \\
&gemini\_1.5\_pro &0.625 &0.329787234042553 &0.597633136094674 &0.653333333333333 &0.533783783783783 &0.706766917293233 &0.661417322834645 &0.463917525773195 &0.738636363636363 &0.545454545454545 &0.653846153846153 &0.444444444444444 \\
&textonly\_llama3\_70b\_8192 &0.351778656126482 &0.260869565217391 &0.476470588235294 &0.579310344827586 &0.363636363636363 &0.36231884057971 &0.507936507936507 &0.316326530612244 &0.609756097560975 &0.54054054054054 &0.528846153846153 &0.404761904761904 \\
\multirow{6}{*}{Few shot} &textonly\_gpt\_3.5\_turbo\_0125 &0.308 &0.325842696629213 &0.209580838323353 &0.478873239436619 &0.305882352941176 &0.311111111111111 &0.300813008130081 &0.294736842105263 &0.367088607594936 &* &0.405940594059405 &0.345679012345679 \\
&gpt\_4o &0.42292490118577 &0.406593406593406 &0.580838323353293 &0.675675675675675 &0.445205479452054 &0.404411764705882 &0.699186991869918 &0.46875 &0.728260869565217 &0.634146341463414 &0.712871287128712 &* \\
&gemini\_1.5\_flash &0.450592885375494 &0.351648351648351 &0.48502994011976 &0.621621621621621 &0.452054794520547 &0.426470588235294 &0.528455284552845 &0.427083333333333 &0.630434782608695 &0.48780487804878 &0.613861386138613 &0.448275862068965 \\
&textonly\_mixtral\_8x7b\_32768 &0.272 &0.247191011235955 &0.281437125748503 &0.507042253521126 &0.294117647058823 &0.274074074074074 &0.333333333333333 &0.294736842105263 &0.189873417721519 &* &0.554455445544554 &0.320987654320987 \\
&gemini\_1.5\_pro &0.632411067193675 &0.373626373626373 &0.592814371257485 &0.689189189189189 &0.602739726027397 &0.683823529411764 &0.585365853658536 &0.4375 &0.804347826086956 &0.634146341463414 &0.702970297029702 &0.620689655172413 \\
&textonly\_llama3\_70b\_8192 &0.34 &0.168539325842696 &0.449101796407185 &0.514084507042253 &0.364705882352941 &0.348148148148148 &0.398373983739837 &0.326315789473684 &0.341772151898734 &* &0.504950495049505 &0.345679012345679 \\
&\multicolumn{13}{c}{Imageonly data} \\
\multirow{5}{*}{Zero shot} &imageonly\_gemini\_1.5\_flash &0.3515625 &0.212765957446808 &0.441176470588235 &0.377483443708609 &0.281879194630872 &0.388489208633093 &0.349206349206349 &0.333333333333333 &0.389473684210526 &0.318181818181818 &0.298076923076923 &0.3 \\
&imageonly\_gemini\_1.5\_pro &0.32421875 &0.319148936170212 &0.476470588235294 &0.523178807947019 &0.275167785234899 &0.37410071942446 &0.38095238095238 &0.292929292929292 &0.473684210526315 &0.477272727272727 &0.384615384615384 &0.444444444444444 \\
&imageonly\_gpt\_4o &0.28125 &0.319148936170212 &0.494117647058823 &0.450331125827814 &0.308724832214765 &0.323741007194244 &0.523809523809523 &0.343434343434343 &0.368421052631578 &0.431818181818181 &0.538461538461538 &0.333333333333333 \\
&imageonly\_internLM &0.18359375 &0.180851063829787 &0.217647058823529 &0.165562913907284 &0.174496644295302 &0.115107913669064 &0.158730158730158 &0.242424242424242 &0.252631578947368 &0.113636363636363 &0.173076923076923 &0.0888888888888888 \\
&imageonly\_qwen &0.296875 &0.234042553191489 &0.264705882352941 &0.23841059602649 &0.275167785234899 &0.231884057971014 &0.182539682539682 &0.262626262626262 &0.305263157894736 &0.0681818181818181 &0.153846153846153 &0.21590909090909 \\
\multirow{5}{*}{Few shot} &imageonly\_gemini\_1.5\_flash &0.272727272727272 &0.263736263736263 &0.443113772455089 &0.405405405405405 &0.260273972602739 &0.286764705882352 &0.300813008130081 &0.302083333333333 &0.369565217391304 &0.24390243902439 &0.336633663366336 &0.298850574712643 \\
&imageonly\_gemini\_1.5\_pro &0.233201581027668 &0.23076923076923 &0.461077844311377 &0.479729729729729 &0.246575342465753 &0.367647058823529 &0.365853658536585 &0.322916666666666 &0.42391304347826 &0.317073170731707 &0.326732673267326 &0.229885057471264 \\
&imageonly\_gpt\_4o &0.320158102766798 &0.296703296703296 &0.502994011976047 &0.425675675675675 &0.321917808219178 &0.352941176470588 &0.430894308943089 &0.25 &0.467391304347826 &0.414634146341463 &0.534653465346534 &0.344827586206896 \\
&imageonly\_internLM & & & & & & & & & & & & \\
&imageonly\_qwen & & & & & & & & & & & & \\
\bottomrule
\end{tabular}
\end{table}

==> tables/table-closed-src-models.tex <==
% \begin{table*}[ht]
% \scriptsize
% \setlength{\tabcolsep}{2.5pt}
% \centering
% \begin{tabular}{lcccccc}
% \toprule
% \textbf{Category} & \textbf{gpt\_4o\_zs} & \textbf{gpt\_4o\_fs} & \textbf{gemini\_1.5\_pro\_zs} & \textbf{gemini\_1.5\_pro\_fs} & \textbf{gemini\_1.5\_flash\_zs} & \textbf{gemini\_1.5\_flash\_fs} \\
% \midrule
% Alphabet Test & 35.11 & 42.55 & 32.98 & 39.36 & 22.34 & 37.23 \\
% Analogy & 65.56 & 68.21 & 65.33 & 69.54 & 56.95 & 62.91 \\
% Blood Relation & 68.25 & 70.63 & 66.14 & 58.73 & 54.76 & 53.97 \\
% Coding-Decoding & 38.26 & 45.64 & 53.38 & 61.07 & 38.26 & 46.31 \\
% Cube and Dice & 35.96 & 40.45 & 45.65 & 43.82 & 32.58 & 31.46 \\
% Data Sufficiency & 43.33 & 0.00 & 44.44 & 63.33 & 42.22 & 46.67 \\
% Direction Sense & 37.50 & 41.67 & 53.06 & 63.54 & 44.79 & 41.67 \\
% Embedded Figure & 22.92 & 0.00 & 24.24 & 36.46 & 25.00 & 36.46 \\
% Figure Partition and Dot Problem & 38.30 & 32.98 & 41.05 & 42.55 & 34.04 & 37.23 \\
% Incomplete Figure & 23.40 & 22.34 & 19.79 & 38.30 & 34.04 & 30.85 \\
% Mathematical Operations & 41.41 & 48.48 & 46.39 & 45.45 & 40.40 & 44.44 \\
% "Mirror, Water and Images" & 34.78 & 0.00 & 34.78 & 35.87 & 28.26 & 28.26 \\
% Missing Character & 29.92 & 29.13 & 37.01 & 37.01 & 25.98 & 29.13 \\
% Non-Verbal Analogy & 26.00 & 0.00 & 26.00 & 32.00 & 32.00 & 35.00 \\
% Non-Verbal Series & 16.84 & 17.89 & 24.49 & 33.68 & 23.16 & 31.58 \\
% Non-Verbal odd one out & 22.86 & 0.00 & 12.33 & 25.71 & 21.43 & 32.86 \\
% Number and Ranking & 42.45 & 41.01 & 70.68 & 68.35 & 39.57 & 41.73 \\
% Odd one out & 55.88 & 58.24 & 59.76 & 60.00 & 48.82 & 49.41 \\
% Paper Folding \& Cutting & 27.08 & 34.38 & 33.33 & 30.21 & 32.29 & 21.88 \\
% Puzzle Test & 69.47 & 73.68 & 73.86 & 81.05 & 60.00 & 62.11 \\
% Series & 42.58 & 42.97 & 62.50 & 63.67 & 36.33 & 45.70 \\
% Statement \& Conclusions & 70.19 & 72.12 & 65.38 & 70.19 & 65.38 & 62.50 \\
% Syllogisms & 63.64 & 65.91 & 54.55 & 65.91 & 63.64 & 52.27 \\
% Time and Clock & 41.18 & 52.94 & 64.15 & 70.59 & 33.33 & 52.94 \\
% Venn Diagrams & 50.45 & 54.05 & 62.26 & 64.86 & 45.05 & 58.56 \\
% \bottomrule
% \end{tabular}
% \caption{Model Performance on Various Categories (Percentage Accuracy) based on interleaving based prompting}
% \label{tab:model_performance_closed}
% \end{table*}
